Controlling Neural Networks with Rule Representations

We propose a novel training method that integrates rules into deep learning, in a way the strengths of the rules are controllable at inference. Deep Neural Networks with Controllable Rule Representations (DeepCTRL) incorporates a rule encoder into the model coupled with a rule-based objective, enabling a shared representation for decision making. DeepCTRL is agnostic to data type and model architecture. It can be applied to any kind of rule defined for inputs and outputs. The key aspect of DeepCTRL is that it does not require retraining to adapt the rule strength -- at inference, the user can adjust it based on the desired operation point on accuracy vs. rule verification ratio. In real-world domains where incorporating rules is critical -- such as Physics, Retail and Healthcare -- we show the effectiveness of DeepCTRL in teaching rules for deep learning. DeepCTRL improves the trust and reliability of the trained models by significantly increasing their rule verification ratio, while also providing accuracy gains at downstream tasks. Additionally, DeepCTRL enables novel use cases such as hypothesis testing of the rules on data samples, and unsupervised adaptation based on shared rules between datasets.

==> related_work.tex <==
\section{Related Work}

Various methods have been studied to incorporate `rules' into deep learning, considering prior knowledge in wide range of applications.
\cite{posteriorreg} shows posterior regularization approach to inject rules into predictions.
In \cite{harnessdnnlogicrules}, a teacher-student framework is used, where the teacher network is obtained by projecting the student network to a (logic) rule-regularized subspace and the student network is updated to balance between emulating the teacher’s output and predicting the true labels. 
\cite{adversarialdebiasing} utilizes adversarial learning specifically for bias rules, to penalize unwanted biases.
Overall, the aforementioned methods lack the flexibility aspect of our approach -- they do not allow controlling the rule strength, in a model- and data-agnostic way.
\cite{fioretto2020lagrangian} proposes a framework that exploits Lagrangian duality to train with rules. 
\cite{pmlr-v84-narasimhan18a} considers learning with constraints via formulation over the space of confusion matrices and optimization solvers that operate through a sequence of linear minimization steps.
\cite{shao2020controlvae} injects a constraints via KL divergence for variational autoencoders, for controlling output diversity or disentangled latent factor representations.
DNN-CRR differentiate from all of the aforementioned methods to inject rules, with the aspect that it allows controllability of the rule strength at the inference without retraining, enabled by accurate learning of the rule representations in the data manifold. This unlocks new capabilities, beyond simply improving rule verification. 

%\citet{higgins2016beta,burgess2018understanding} propose an adjustable hyperparameter $\beta$ to balance between KL divergence and a reconstruction error in VAE and 


